Automated proof synthesis for propositional logic with deep neural networks

This work explores the application of deep learning, a machine learning technique that uses deep neural networks (DNN) in its core, to an automated theorem proving (ATP) problem. To this end, we construct a statistical model which quantifies the likelihood that a proof is indeed a correct one of a given proposition. Based on this model, we give a proof-synthesis procedure that searches for a proof in the order of the likelihood. This procedure uses an estimator of the likelihood of an inference rule being applied at each step of a proof. As an implementation of the estimator, we propose a proposition-to-proof architecture, which is a DNN tailored to the automated proof synthesis problem. To empirically demonstrate its usefulness, we apply our model to synthesize proofs of propositional logic. We train the proposition-to-proof model using a training dataset of proposition-proof pairs. The evaluation against a benchmark set shows the very high accuracy and an improvement to the recent work of neural proof synthesis.

==> sec/onFinitenessNormal.tex <==

\section{Texts to be used somewhere}

% We restrict the proof terms in the training set to $\beta\eta$-normal
% ones.  We partially justify this choice in the following.

\subsection{Duplicate-free normal forms}

\KS{State here that the distribution we are trying to learn is
  degenerate if we allow all the terms.}  As we mentioned in
Section~\ref{}, our network is intended to learn the following
distribution:
\[
  p(\_ \mid \_)
\]

Our choice of limiting the proof terms to be normal forms is
admittedly pragmatic; if we did not impose this condition, then the
distribution~\ref{def:distributionToBeLearned} is sometimes degenerate
as the following example suggests.
\begin{example}
  Let $\Gamma := s : \mathit{a} \,  \mathord{\rightarrow}  \, \mathit{a}, x : \mathit{a}$ and $\tau := \mathit{a}$.  Then,
  the following set of terms are all proofs of $\tau$ under $\Gamma$:
  \[
    \begin{array}{l}
      \left\{ x \right\} \cup\\
      \left\{ x \right\} \cup \cdots
    \end{array}
  \]
\end{example}
Therefore, if we allow all the proof terms to be considered in
defining the distribution~\ref{def:distributionToBeLearned}, it is in
general impossible to learn a meaningful automated theorem prover from
data.

We resolve this issue by limiting the set of the proof terms in the
definition of the distribution.  Concretely, we allow only the
following \emph{duplicate-free normal proof} in defining the
distribution.
\begin{definition}
  \label{def:duplicateFreeNormal}
  Proof term $M$ is said to be \emph{duplicate-free normal proof}
  under $\Gamma$ and $\tau$ if (1) $\Gamma \vdash M : \tau$, (2) $M$
  is $\eta$-long normal, and (3) the derivation tree of
  $\Gamma \vdash M : \tau$ does not contain any path of the following
  form: \[\dots\]

  We write $\DupFreeNormal{\Gamma}{\tau}$ for the set of the
  duplicate-free normal proofs under $\Gamma$ and $\tau$.
\end{definition}

The following lemma justifies the limitation to the duplicate-free
normal proofs instead of the general proof terms.
\begin{lemma}
  \label{lem:completenessDupFree}
  \KS{To be proved.}  If there exists $M$ such that
  $\Gamma \vdash M : \tau$, then there is
  $P \in \DupFreeNormal{\Gamma}{\tau}$ such that
  $\Gamma \vdash P : \tau$.
\end{lemma}
Moreover, the following lemma guarantees that
$\DupFreeNormal{\Gamma}{\tau}$ is finite for any $\Gamma$ and $\tau$;
hence, the distribution defined over $\DupFreeNormal{\Gamma}{\tau}$ is
not degenerate.
\begin{lemma}
  \label{lem:dupFreeNormalFinite}
  \KS{To be proved.}  The set $\DupFreeNormal{\Gamma}{\tau}$ is finite
  for any $\Gamma$ and $\tau$.
\end{lemma}

%% We learn the following probabilistic distribution.
%% \[
%% p(M | \Gamma,\tau)
%% \]

